Ambient Sound Provides Supervision for Visual Learning

The sound of crashing waves, the roar of fast-moving cars -- sound conveys important information about the objects in our surroundings. In this work, we show that ambient sounds can be used as a supervisory signal for learning visual models. To demonstrate this, we train a convolutional neural network to predict a statistical summary of the sound associated with a video frame. We show that, through this process, the network learns a representation that conveys information about objects and scenes. We evaluate this representation on several recognition tasks, finding that its performance is comparable to that of other state-of-the-art unsupervised learning methods. Finally, we show through visualizations that the network learns units that are selective to objects that are often associated with characteristic sounds.

==> tbl-psychophysics.tex <==
\begin{table}[t]
  \centering
  \begin{tabular}{lc}
    \toprule
    Method  &  Labeled Real \\
    \midrule
    \model (cluster)  & 38.4\% \\
    \model (binary) &  29.4\%  \\
    ImageNet~\cite{krizhevsky2012imagenet}  &    37.8\% \\
    Random & 24.0\% \\
    \bottomrule
  \end{tabular}
  \vspace{5pt}
  \caption{Percentage of synthesized sound labeled as real (chosen over the ground-truth sound) by human subjects in a real-or-fake study (higher is better).}
  \label{tbl:syn}
\end{table}

